VeCLIP: Improving CLIP Training via Visual-enriched Captions

Large-scale web-crawled datasets are fundamental for the success of pre-training vision-language models, such as CLIP. However, the inherent noise and potential irrelevance of web-crawled AltTexts pose challenges in achieving precise image-text alignment. Existing methods utilizing large language models (LLMs) for caption rewriting have shown promise on small, curated datasets like CC3M and CC12M. This study introduces a scalable pipeline for noisy caption rewriting. Unlike recent LLM rewriting techniques, we emphasize the incorporation of visual concepts into captions, termed as Visual-enriched Captions (VeCap). To ensure data diversity, we propose a novel mixed training scheme that optimizes the utilization of AltTexts alongside newly generated VeCap. We showcase the adaptation of this method for training CLIP on large-scale web-crawled datasets, termed VeCLIP. Employing this cost-effective pipeline, we effortlessly scale our dataset up to 300 million samples named VeCap dataset. Our results show significant advantages in image-text alignment and overall model performance. For example, VeCLIP achieves up to +25.2% gain in COCO and Flickr30k retrieval tasks under the 12M setting. For data efficiency, VeCLIP achieves +3% gain while only using 14% of the data employed in the vanilla CLIP and 11% in ALIGN. We also note the VeCap data is complementary with other well curated datasets good for zero-shot classification tasks. When combining VeCap and DFN, our model can achieve strong performance on both of image-text retrieval and zero-shot classification tasks, e.g. 83.1% accuracy@1 on ImageNet zero-shot for a H/14 model. We release the pre-trained models at https://github.com/apple/ml-veclip.

==> Tables/Ablation_2.tex <==
\begin{table}[t]
    \centering
    \caption{\small{ Ablation studies on captions. . 
}}
    \vspace{-0.2cm}
    \small
    \resizebox{1.0\textwidth}{!}{
\begin{tabular}{cccc|ccccc}
\toprule[1.2pt]
\multirow{2}{*}{\bf Data} & \multirow{2}{*}{\bf Caption} & \multirow{2}{*}{\thead{ \bf Prompt \\ Constraint}  } & \multirow{2}{*}{\thead{ \bf Caption \\ Sampling}} & \multicolumn{2}{c}{ \bf COCO (R@1)} & \multicolumn{2}{c}{\bf Flickr30k (R@1)} & \multirow{2}{*}{ \bf ImageNet} \\
                  &    &    &    &  I-T  & T-I  &  I-T & T-I   &            \\
\midrule     
\multirow{4}{*}{3M} &                   &                   &                   &           &          &           &          &                   \\
                  &                   &                   &                   &           &          &           &          &                   \\
                  &                   &                   &                   &           &          &           &          &                   \\
                  &                   &                   &                   &           &          &           &          &   \\
\bottomrule[1.2pt]
\end{tabular}
    }
    % \caption{Caption}
    \label{tab:abla_caption}
\end{table}

==> Tables/Retrieval.tex <==
\begin{table*}[t]
    \centering
    \caption{\small{ Results (Recall@$k$) on zero-shot image-to-text and text-to-image retrieval tasks on COCO and Flickr30k. 1.4B-CLIP denotes the in-house CLIP pre-trained on 1.4B web-crawled image-text pairs. We use ViT-B/16 as the vision encoder of CLIP. (*) FLIP uses ViT-L/14. 
}}
    \vspace{-0.2cm}
    \small
    \resizebox{1.0\textwidth}{!}{
    \begin{tabular}{lc|cccccc|cccccc}
  
    \toprule[1.2pt]
    \multirow{3}{*}{\bf Data} & \multirow{3}{*}{\bf Model} & \multicolumn{6}{c|}{\bf COCO}                        & \multicolumn{6}{c}{\bf Flickr30k}    \\                     
    &                   & \multicolumn{3}{c}{ \bf Image-to-Text} & \multicolumn{3}{c|}{\bf Text-to-Image} & \multicolumn{3}{c}{\bf Image-to-Text} & \multicolumn{3}{c}{\bf Text-to-Image} \\
    &                   &  R@1     &   R@5    &  R@10    &   R@1    &     R@5   &  R@10    &  R@1     &   R@5    &  R@10    &   R@1    &     R@5   &  R@10       \\
    
    % & &  Caltech101 & CIFAR100 & SVHN & DTD & OxPet & Flowers102 & Eurosat & RESISC60 & Camelyon \\
 
    \midrule 
    \small 
    \bf 1.8B & \small ALIGN~\citep{ALIGN} & 58.60 & 83.00 & 89.70 & 45.60 & 69.80 & 78.60 & 88.60 & \bf 98.70 & \bf 99.70 & 75.70 & \bf 93.80 & \bf 96.80 \\
    \bf 400M & \small FLIP*~\citep{flip} & 60.20 & 82.60 & 89.90 & 44.20 & 69.20 & 78.40 & 89.10 & 98.50 & 99.60 & 75.40 & 92.50 & 95.90 \\
    \midrule
    \bf 400M & \small  OpenAI CLIP & 53.76 & 77.92 & 85.53 & 33.09 & 58.42 & 68.90 & 88.00 & \bf 98.70 & 99.40 & 68.70 & 90.60 & 95.20 \\
    \bf 1.4B & \small In-house CLIP & 61.38	& 82.80 &	89.78	&44.48	&69.19 &	78.28
    & 87.60	& 97.90	& 98.80 &	71.70	& 91.30	& 95.24 \\
    \midrule
    
    \multirow{2}{*}{\bf 3M} & \small CLIP & 5.46	&15.34	&22.42	&3.28	&10.44	& 15.96 & 12.20	& 27.80	& 37.50	& 6.36	&19.16	&27.58  \\
    &  \small VeCLIP & \bf 22.30	& \bf 45.00 & \bf	56.16 & \bf	13.01 &	\bf 31.61	& \bf 42.42 & \bf 40.60	& \bf 67.30	& \bf 76.70	& \bf 27.58 & 	\bf 52.44 & 	\bf 63.20 \\
    % \rowcolor{tbgray}  \multicolumn{2}{c|}{\bf Performance Gain} & \bf \textcolor{green}{+16.84}	& \bf \textcolor{green}{+29.66}	& \bf \textcolor{green}{+33.74}	& \bf \textcolor{green}{+9.73} 	& \bf \textcolor{green}{+21.17}	& \bf \textcolor{green}{+26.46} & \bf \textcolor{green}{+28.40}	& \bf \textcolor{green}{+39.50}	& \bf \textcolor{green}{+39.20}	& \bf \textcolor{green}{+21.22} & \bf \textcolor{green}{+33.28}	& \bf \textcolor{green}{+35.62} \\

    \midrule 
    \multirow{2}{*}{\bf 12M} & \small CLIP & 24.52	& 48.28	& 59.82 &	14.28	& 34.52 &	46.29 & 44.70	& 71.80 &	80.40 &	29.06	& 58.62 &	70.00 \\
    &  \small VeCLIP & \bf 47.78	& \bf 72.54	& \bf 81.56	& \bf 31.62	& \bf 57.19	& \bf 68.47 & \bf 73.90	& \bf 92.30	& \bf 95.90	& \bf 55.68	& \bf 80.78	& \bf 87.64 \\
    % \rowcolor{tbgray}  \multicolumn{2}{c|}{\bf Performance Gain} & \bf \textcolor{green}{+23.26}	& \bf \textcolor{green}{+24.26}	& \bf \textcolor{green}{+21.74}	& \bf \textcolor{green}{+17.34} 	& \bf \textcolor{green}{+22.67}	& \bf \textcolor{green}{+22.18} & \bf \textcolor{green}{+29.20}	& \bf \textcolor{green}{+20.50}	& \bf \textcolor{green}{+15.50}	& \bf \textcolor{green}{+26.62} & \bf \textcolor{green}{+22.16}	& \bf \textcolor{green}{+17.64} \\
    \midrule 
    \multirow{2}{*}{\bf 100M} & \small CLIP & 47.24	&72.34	&81.56&	30.61	& 56.49	& 67.91 & 74.40	& 93.20	& 96.70 &	57.16 & 	88.12 &	88.98\\
    &  \small VeCLIP &\bf   64.82	& \bf 85.56& \bf 91.98	& \bf 46.12	& \bf 71.19	& \bf 80.23 & \bf  89.30	& \bf   97.70	& \bf  99.20 &	\bf  73.10	& \bf  89.12	& \bf 93.14 \\
    % \rowcolor{tbgray}  \multicolumn{2}{c|}{\bf Performance Gain} & \bf \textcolor{green}{+17.58}	& \bf \textcolor{green}{+13.22}	& \bf \textcolor{green}{+10.42}	& \bf \textcolor{green}{+15.51} & \bf \textcolor{green}{+14.70}	& \bf \textcolor{green}{+12.32} & \bf \textcolor{green}{+14.90}	& \bf \textcolor{green}{+4.50}	& \bf \textcolor{green}{+2.50}	& \bf \textcolor{green}{+15.94} & \bf \textcolor{green}{+1.00}	& \bf \textcolor{green}{+4.16} \\
    \rowcolor{tbgray}  \multicolumn{2}{c|}{\bf Performance Gain vs 1.4B-CLIP} & \bf \textcolor{green}{+3.44}	& \bf \textcolor{green}{+2.76}	& \bf \textcolor{green}{+2.20}	& \bf \textcolor{green}{+1.64} & \bf \textcolor{green}{+2.00}	& \bf \textcolor{green}{+1.95} & \bf \textcolor{green}{+1.70}	& \bf \textcolor{red}{-0.20}	& \bf \textcolor{green}{+0.40}	& \bf \textcolor{green}{+1.60} & \bf \textcolor{red}{-2.18}	& \bf \textcolor{red}{-2.10} \\
   
    
    \midrule 
    \multirow{2}{*}{\bf 200M} & \small CLIP &  52.20	& 76.22	& 85.04	& 34.97	& 60.42	& 71.08 & 80.90	& 94.90	& 97.60	& 63.26 &	86.58	& 92.26 \\
    &  \small VeCLIP & \bf 67.20	& \bf 87.28 &  \bf	92.70	& \bf 48.40	& \bf 73.26 & \bf	81.79 &  \bf 91.10 &	 \bf 98.50 & \bf	99.70	& \bf 76.32	& \bf 93.50	& \bf 96.40 \\
    % \rowcolor{tbgray}  \multicolumn{2}{c|}{\bf Performance Gain} & \bf \textcolor{green}{+15.00}	& \bf \textcolor{green}{+11.06}	& \bf \textcolor{green}{+7.66}	& \bf \textcolor{green}{+13.43} & \bf \textcolor{green}{+12.84}	& \bf \textcolor{green}{+10.71} & \bf \textcolor{green}{+10.20}	& \bf \textcolor{green}{+3.60}	& \bf \textcolor{green}{+2.10}	& \bf \textcolor{green}{+13.06} & \bf \textcolor{green}{+6.92}	& \bf \textcolor{green}{+4.14} \\
    % \hline[dashed]
    % \hdashline

    \rowcolor{tbgray}  \multicolumn{2}{c|}{\bf Performance Gain vs 1.4B-CLIP} & \bf \textcolor{green}{+5.82}	& \bf \textcolor{green}{+4.48}	& \bf \textcolor{green}{+2.92}	& \bf \textcolor{green}{+3.92} & \bf \textcolor{green}{+4.07}	& \bf \textcolor{green}{+3.51} & \bf \textcolor{green}{+3.50}	& \bf \textcolor{green}{+0.60}	& \bf \textcolor{green}{+0.90}	& \bf \textcolor{green}{+4.62} & \bf \textcolor{green}{+2.20}	& \bf \textcolor{green}{+1.16} \\
   
    % \midrule
    % % \hline
    % \multirow{2}{*}{\bf 12M} & \small CLIP & 70.43 & 30.06 & 30.11 & 30.69 & 34.51 & 33.67 & 8.87 & 30.05 & 53.46 & 35.76 \\
    % & \small VeCLIP & \bf 70.58 & \bf 45.10 & \bf 23.61 & \bf 30.90 & \bf 36.22 & \bf 43.94 & \bf 27.46 & \bf 38.09 & \bf 55.54 & \bf 41.27  \\
    % \midrule
    % % \hline
    % \multirow{2}{*}{\bf 100M} & \small CLIP & 81.44 & 54.75 & 38.70 & 57.28 & 70.51 & 51.71 & 34.45 & 48.56 & 53.87 & 54.59  \\
    % & \small VeCLIP & \bf 81.64 & \bf 64.62 & \bf 46.49 & \bf 57.51 & \bf  64.81 & \bf 66.41 & \bf 46.23 & \bf 51.75 & \bf 58.51 & \bf 59.78   \\


    
    
         % &  \\
         % & 
    \bottomrule[1.2pt]
    \end{tabular}
    }
    % \vspace{-0.4cm}
    % \caption{Caption}
    \label{tab:retrieval}
\end{table*}

==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}


